ARTiST: Automated Text Simplification for Task Guidance in Augmented Reality

Text presented in augmented reality provides in-situ, real-time information for users. However, this content can be challenging to apprehend quickly when engaging in cognitively demanding AR tasks, especially when it is presented on a head-mounted display. We propose ARTiST, an automatic text simplification system that uses a few-shot prompt and GPT-3 models to specifically optimize the text length and semantic content for augmented reality. Developed out of a formative study that included seven users and three experts, our system combines a customized error calibration model with a few-shot prompt to integrate the syntactic, lexical, elaborative, and content simplification techniques, and generate simplified AR text for head-worn displays. Results from a 16-user empirical study showed that ARTiST lightens the cognitive load and improves performance significantly over both unmodified text and text modified via traditional methods. Our work constitutes a step towards automating the optimization of batch text data for readability and performance in augmented reality.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> hackstyle.tex <==
%\setlength{\titlespace}{0ex}
%\setlength{\titlespace}{1.0ex}
%\setlength{\textheight}{9.25in}
\setlength{\abovecaptionskip}{1.0ex}
\setlength{\belowcaptionskip}{1.0ex}
\setlength{\floatsep}{1.0ex}
\setlength{\dblfloatsep}{\floatsep}
\setlength{\textfloatsep}{2.0ex}
\setlength{\dbltextfloatsep}{\textfloatsep}
%\setlength{\intextsep}{1.0ex}
\setlength{\abovedisplayskip}{1.0ex}
\setlength{\belowdisplayskip}{1.0ex}
%\setlength{\arraycolsep}{1ex}
%\setlength{\parskip}{1.0ex} % actually increase space for acmart
%\setlength{\baselineskip}{1ex}
%\setlength{\teaserspace}{1ex}
%\linespread{1.0} % default 1.0; WMD! very evil, be very careful


==> iceberg/method.tex <==
\section{Method}
Based on the extracted guidelines from the formative study, we propose a automated text simplification system for the augmented reality. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/sys.pdf}
    \caption{System Overview}
    \label{fig:one-column}
\end{figure*}

\subsection{Infrastructure}
Our system is designed to provide augmented reality (AR) task guidance for users utilizing the Microsoft HoloLens platform. The system is comprised of three primary components: a manual management system for remote experts, a text simplification engine based on established design guidelines, and a front-end text display interface integrated with Microsoft HoloLens. The manual management system facilitates the process of manual input by developers through a web-based interface. Once the task manual is input, it is transmitted to the text simplification engine for online processing. This engine employs object detection techniques to identify pertinent objects within the user's field of view and leverages OpenAI's GPT- model via zero-shot learning to generate a simplified version of the text. Subsequently, the simplified text is made available on the manual management system, allowing remote experts to review and verify the results. Finally, the refined text is displayed on the Microsoft HoloLens interface, enhancing the user experience and facilitating task guidance in real-time.

\subsection{Manual Management}
The manual management system serves as a centralized platform for inputting, storing, and processing the task manuals, allowing remote experts and developers to collaborate on creating and refining task guidance. 
The prototype supports the four 
The manual management system also offers version control, facilitating the tracking of changes and allowing for easy retrieval of previous versions if necessary. Additionally, the system supports various file formats and allows for manual organization through tagging, categorization, and search functionality. This ensures that the repository of task manuals remains accessible, well-structured, and easily navigable for all stakeholders involved in the development and maintenance of AR task guidance.


\subsection{Text Simplification Engine}
The text simplification engine is the core component of our system, responsible for transforming complex task manuals into concise, AR-friendly instructions. This engine incorporates the design guidelines derived from the formative study, ensuring that the resulting simplified text is tailored for AR users. The engine first performs object detection to identify relevant objects in the user's field of view. This is achieved through a combination of computer vision techniques and pre-trained object detection models. The identified objects are then used to contextualize and adapt the task manual to the user's environment.
[]




\subsubsection{Hololens Interface}
The HoloLens interface serves as the front-end display for users, presenting the simplified text and other relevant information during task guidance. As a critical component of our system, the interface has been designed to maximize usability and minimize cognitive load for the user while they interact with the AR environment.

The interface layout is organized into distinct, easily discernible visual elements, ensuring that users can quickly locate and comprehend the information they need. The simplified text is displayed prominently, with a font size and style that is easily readable in the AR context. The color palette, as mentioned earlier, is chosen to provide good contrast and visibility while maintaining an elegant and academic appearance.

Spatial anchoring is employed to position the text and other interface elements relative to the user's field of view and the identified objects in the environment. This ensures that the task guidance remains visible and accessible, even as the user moves around and interacts with the AR environment. The interface also supports dynamic adjustment of its position and orientation based on user preferences and real-time tracking of the user's head movements.

To further enhance the user experience, the HoloLens interface incorporates voice commands and gesture recognition, allowing users to interact with the system in a more intuitive and natural way. Users can issue commands to navigate through the task guidance, request additional information, or control the display of the interface. Gesture recognition enables users to perform actions such as pointing at objects or making hand gestures to interact with the system.

The HoloLens interface is designed to be easily customizable and adaptable, allowing developers and remote experts to adjust the display and interaction options to suit the specific needs of the users and




==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> meta/authors.tex <==
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Guande Wu}
\email{guandewu@nyu.edu}
\orcid{0000-0002-9244-173X}
% \author{Jing Qian}
% \orcid{0000-0002-5517-3035}
% \email{jq2267@nyu.edu}
% \author{Sonia Castelo}
% \email{s.castelo@nyu.edu}
% \orcid{0000-0001-6881-3006}

\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}

\author{Jing Qian}
\orcid{0000-0002-5517-3035}
\email{jq2267@nyu.edu}
\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}

\author{Sonia Castelo}
\email{s.castelo@nyu.edu}
\orcid{0000-0001-6881-3006}
\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}


\author{Shaoyu Chen}
\orcid{0000-0002-1856-6294}
\email{sc6439@nyu.edu}
\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}


\author{Joao Rulff}
\email{jlrulff@nyu.edu}
\orcid{0000-0003-3341-7059}
\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}

\author{Claudio Silva}
\email{csilva@nyu.edu}
\orcid{0000-0003-2452-2295}
\affiliation{%
  \institution{New York University}
  \streetaddress{370 Jay St.}
  \city{Brooklyn}
  \state{New York}
  \country{USA}
  \postcode{11201}
}

==> meta/commands.tex <==

% \newcommand{\systemname}{TSimer~}

\newcommand{\systemname}{ARTiST}


\newcommand{\mytodo}[1]{\colorbox{red!25}{\textcolor{white}{TODO: #1}}}

\newcommand{\textquote}[1]{\textit{#1}}

\newcommand{\sampletext}[1]{\textit{#1}}
\newcommand{\simplificationWay}[1]{A#1}
\newcommand\myparagraph[1]{\textit{#1.}~}
\newcommand\myparagraphbold[1]{ \noindent \textbf{#1}}

\newcommand\myheading[1]{ \textbf{#1}}

% \newcommand{\revision}[2]{\sout{#1} \textcolor{blue}{#2}}
% \newcommand{\revision}[2]{ \textcolor{blue}{#2}}
% \newcommand\revblue[1]{\textcolor{blue}{#1}}

% \newcommand{\revision}[2]{{#2}}
% \newcommand\revblue[1]{{#1}}
\newcommand\revblue[1]{{#1}}

% \newcommand\revisionbluetext[1]{{#1}}
\newcommand\revisionbluetext[1]{\textcolor{blue}{#1}}


\newcommand{\guande}[1]{\textcolor[HTML]{FFC0CB}{[Guande: #1]}} % John's color
\newcommand{\jing}[1]{\textcolor[HTML]{228B22}{[Jing: #1]}} % Jane's color
\newcommand{\joao}[1]{\textcolor[HTML]{B22222}{[Joao: #1]}} % Alex's color
\newcommand{\sonia}[1]{\textcolor[HTML]{DDA0DD}{Sonia: [#1]}} % Maria's color
\newcommand{\shaoyu}[1]{\textcolor[HTML]{CC5500}{[Shaoyu: #1]}} % David's color
\newcommand{\claudio}[1]{\textcolor[HTML]{008080}{[Claudio: #1]}} % Susan's color

\newcommand{\participantquote}[1]{``\textit{#1}''}
\newcommand{\instructionquote}[1]{\textit{#1}}


==> tables/study1-task1-sample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[ht]
\begin{tabular}{|r|p{6cm}|p{6cm}|}
\hline
\multicolumn{1}{|l|}{Step} & Original                                                                                                                                                                                                     & Simplification                                                                                                \\ \hline
1                          & To create a coffee, first please carefully place the pour-over dripper over the coffee mug.                                                                                                                  & { Place dripper (on your left) on coffee mug.}                                            \\ \hline
2                          & Prepare the filter insert by folding the paper filter in half to create a semi-circle, and in half again to create a quarter-circle. Place the paper filter in the dripper and spread open to create a cone. & { Fold paper filter in half, then half again. Put filter in dripper, form cone shape.}    \\ \hline
3                          & Rinse the filter. Pour enough hot water into the filter to wet it. The entire paper filter should be moist. Rinsing the filter will remove any papery residue so your coffee doesn't have a woodsy taste.    & { Wet filter with water to rinse away residue.}                                           \\ \hline
4                          & Lift up the dripper and pour out the water. Then set the dripper with the wet filter back on the coffee mug.                                                                                                 & { Remove dripper, pour out water, and return dripper to coffee mug.}                      \\ \hline
5                          & Get out a digital scale and measure out 3 tablespoons (about 30 g) of coffee beans. Measure out 30 g of whole beans and place them in your grinder.                                                          & { Measure 30g coffee beans on a digital scale (right side), place in grinder (right side).} \\ \hline
6                          & Grind the beans until the coffee grounds are the consistency of coarse sand, about 20 seconds.                                                                                                               & { Grind beans for 20 seconds, until coarse sand consistency.}                             \\ \hline
7                          & Transfer the coffee grounds to the filter cone. Then place the coffee mug with the dripper on a digital scale and set it to zero.                                                                            & { Move grounds to filter cone. Set coffee mug with dripper on scale, zero it.}            \\ \hline
8                          & Slowly pour the water over the grounds in a circular motion. Do not overfill beyond the top of the paper filter. Your scale should read 100 g once you've poured enough water into the dripper.              & { Slowly pour water in circles over grounds, stopping at 100g on scale.}                  \\ \hline
9                          & Let the coffee drain completely into the mug and wait for 30 seconds and you can complete the task;                                                                                  & { Drain coffee into mug and wait for 30 seconds to end.}                                  \\ \hline
\end{tabular}
\caption{Study 1 task 1 sample result. The original and simplified versions of the text are listed. The sample is collected from P10's experiment session and the simplified results for other participants may vary slightly due to spatial context.}
\label{tab:study1-task1-samples}
\end{table*}

==> tables/study1-task2-sample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[ht]
\begin{tabular}{|r|p{6cm}|p{6cm}|}
\hline
\multicolumn{1}{|l|}{Step} & Original                                                                                                                                                                                                                                  & Simplification                                                                                                                                       \\ \hline
1                          & Before arranging the meeting room, take a moment to tidy up the desk and move anything that's not necessary to other desks;                                                                                       & Tidy desk, move the unnecessary items to other desks.                                                                        \\ \hline
2                          & Once the desk is clear, bring the power strip on the desk and connect the Charger to the power strip so the meeting attendants can use.                                                                           & Put power strip on desk, connect phone charger to it.                                                                        \\ \hline
3                          & Connect the camera's charger to the power strip and position the camera at the opposite end of the desk from the TV.                                                                                              & Connect camera to strip, facing opposite of TV.                                                                              \\ \hline
4                          & Arrange the chairs in the meeting room. Make sure that there's enough space between each chair - roughly 1.5 feet should suffice. Position one chair on the window side, and place five chairs on the other side. & Arrange chairs on two sides. Leave space of roughly two A4 papers' length apart. Window side: 1 chair. Other side: 5 chairs. \\ \hline
5                          & Next, place cups of water and papers on each chair. Each person should have one cup of water and paper;                                                                                                           & Place water, paper onto desk in front of chairs.                                                                             \\ \hline
6                          & Put up the desk nameplates on on each chair. When Alice is on the side of the window, other desk nameplates should be put on the other side. The sequence is Bob, Amy, Andy, Dave and Luis.                       & Place nameplates: Window side: Alice (window); sequence (left to right) on other side: Bob, Amy, Andy, Dave, Luis.           \\ \hline
7                          & Since Alice is the VIP in the meeting, place make it clearly by putting the remote controller to Alice’s position.                                                                                                & Place remote controller at Alice’s position on desk.                                                                         \\ \hline
\end{tabular}
\caption{Study 1 task 2 sample result. The original and simplified versions of the text are listed. The sample is collected from P10's experiment session and the simplified results for other participants may vary slightly due to spatial context.}
\label{tab:study1-task2-samples}

\end{table}
